Out of Sight, Still in Mind: Reasoning and Planning about Unobserved Objects with Video Tracking Enabled Memory Models

Robots need to have a memory of previously observed, but currently occluded objects to work reliably in realistic environments. We investigate the problem of encoding object-oriented memory into a multi-object manipulation reasoning and planning framework. We propose DOOM and LOOM, which leverage transformer relational dynamics to encode the history of trajectories given partial-view point clouds and an object discovery and tracking engine. Our approaches can perform multiple challenging tasks including reasoning with occluded objects, novel objects appearance, and object reappearance. Throughout our extensive simulation and real-world experiments, we find that our approaches perform well in terms of different numbers of objects and different numbers of distractor actions. Furthermore, we show our approaches outperform an implicit memory baseline.

==> overview_fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle%
\renewcommand{\@maketitle}{\@oldmaketitle%
  \begin{center}
    \centering
    \vspace{-10pt}
    \includegraphics[width=\textwidth]{figures/figure_1_multi_compressed.pdf}
    \vspace{-24pt}
  \end{center}
  \footnotesize{\textbf{Fig.~\thefigure:\label{fig:overview_figure}}~\textbf{Planning using our memory models:} We show several examples of how our model can achieve desired goal relations including unobserved objects, novel objects' appearance and reappearance. We provide a detailed explanation of this figure in section.~\ref{sec:quantitative}.}
  \vspace{-20pt}
  \medskip}
\makeatother
\shrinka
\maketitle
\shrinka
\thispagestyle{empty}
\pagestyle{empty}



==> preliminary.tex <==
We provide the background information here about the transformers, which is the core component of our approaches. 
Transformers, an attention-based approach, are proposed in ~\cite{vaswani2017attention} for sequential data.
A transformer takes the input as a sequence $N$ with length \(n\) and the output is another sequence $\hat{N}$ with the same sequence length \(n\).
The heart of the transformer is the attention between different nodes in the sequence $N$.  
Given each input feature $N_i$, it will be linearly projected to a query, key, and value. 
The function to compute attention is $\texttt{Attention}(Q,K,V) = \texttt{softmax}(\frac{QK^{T}}{\sqrt{d_{k}}})V$, where $d_k$ is the dimension of queries $Q$.
Then the output $\hat{N_{i}}$ is a weighted sum of values based on computed attention.
Furthermore, we can use $k$ layers of the transformer blocks for the input $N$ to get deep features. 
We used an encoder of the transformer in this paper. 
We refer you to the original paper ~\cite{vaswani2017attention} for more details about the transformers. 
